TANGO: Training-free Embodied AI Agents for Open-world Tasks

Large Language Models (LLMs) have demonstrated excellent capabilities in composing various modules together to create programs that can perform complex reasoning tasks on images. In this paper, we propose TANGO, an approach that extends the program composition via LLMs already observed for images, aiming to integrate those capabilities into embodied agents capable of observing and acting in the world. Specifically, by employing a simple PointGoal Navigation model combined with a memory-based exploration policy as a foundational primitive for guiding an agent through the world, we show how a single model can address diverse tasks without additional training. We task an LLM with composing the provided primitives to solve a specific task, using only a few in-context examples in the prompt. We evaluate our approach on three key Embodied AI tasks: Open-Set ObjectGoal Navigation, Multi-Modal Lifelong Navigation, and Open Embodied Question Answering, achieving state-of-the-art results without any specific fine-tuning in challenging zero-shot scenarios.

==> preamble.tex <==
%
% --- inline annotations
%
\newcommand{\red}[1]{{\color{red}#1}}
\newcommand{\todo}[1]{{\color{red}#1}}
\newcommand{\TODO}[1]{\textbf{\color{red}[TODO: #1]}}
% --- disable by uncommenting  
% \renewcommand{\TODO}[1]{}
% \renewcommand{\todo}[1]{#1}



==> sec/intro.tex <==
\section{Introduction}
\label{sec:intro}
%%BOZZA PRIMA IMMAGINE
\begin{figure}[ht]
\begin{center}
\includegraphics[width=.5\textwidth]{sec/images_new/teaser.pdf}
\caption{We introduce \textbf{\approach}, a modular neuro-symbolic system for compositional embodied visual navigation. Given a few examples of natural language instructions and the desired programs, \approach\ is able to generate a program which is then executed by the agent in the environment using a PointGoal Navigation model as its foundational primitive. This figure shows an example (top) in which \approach\ successfully synthesizes a program for the ObjectNav task, as well as an example (bottom) for Embodied QA.}
\label{img:teaser}
\vspace{-10pt}
\end{center}
\end{figure}

Large Language Models (LLMs) have gained significant attention in the field of AI, commended for their impressive ability to generalize and produce responses akin to human reasoning \cite{gpt, team2023gemini, jiang2023mistral, touvron2023llama}. 
These generalization capabilities have been recently exploited to tackle complex visual tasks given, as an input to the model, natural language instructions, thus providing a general and modular interface for a broad range of compositional problems. 
This is the key contribution of frameworks such as VisProg~\cite{visprog} and ViperGPT~\cite{vipergpt} that are able to generate new programs (e.g. Python code) combining a set of predefined off-the-shelf computer vision models and basic routines (like logical operators), by effectively exploiting the in-context learning ability of LLMs like GPT-3~\cite{gpt}.
Previously, methods such as Neural Module Networks (NMN)~\cite{nmn2016,hu2017learning} have demonstrated promising compositional properties for high level tasks like visual question answering, via end-to-end training of networks and specialized, differentiable neural modules. However, they required the combination of semantic parsers and predefined templates to learn to solve the compositional tasks. 
%\FZ{ Alternative approaches, such as those presented in~\cite{nav-gpt2, nav-gpt}, leverage the reasoning capabilities of large language models (LLMs); however, they lack a modular structure that allows for further extensibility or integration.}
In contrast, VisProg and ViperGPT~\cite{visprog,vipergpt} demonstrated strong performance on a broad range of  vision-and-language tasks by just relying on a few number of in-context examples to generate complex programs without requiring any specific training.
Nevertheless, the evaluation of these systems has primarily focused on images in a static scenario. %, neglecting temporal considerations and the potential for executing actions based on an agent's perceptions—essential elements for addressing challenges in navigation or manipulation. 


This paper takes a significant stride in extending the key idea introduced in these seminal works, for the highly dynamic domain of Embodied AI (EAI)~\cite{deitke2022retrospectives}, by defining specialized modules tailored for visual navigation tasks.
Recent years have witnessed a significant growth in interest in EAI, fueled by the emergence of high-frame-rate simulators such as Habitat and iGibson~\cite{savva2019habitat, shen2021igibson, kolve2017ai2}. These simulators have ushered in a new era, fostering models based on end-to-end reinforcement learning that have been able to obtain impressive performance on tasks such as PointGoal Navigation, in which an agent navigates from one point to another within an environment~\cite{wijmans2019dd}. 
However, when faced with more semantically intricate tasks like ObjectGoal Navigation~\cite{chaplot2020object, ye2021auxiliary, batra2020objectnav}, or those requiring long-term memory and strategic planning such as MultiObjectNavigation~\cite{multion, mopa}, modular approaches have proven successful. These often leverage pre-trained components based on mapping and path planning, over generated maps~\cite{chaplot2020learning, chaplot2020object, krantz2023navigating, mopa}.
However, while being very effective for a specific task, these modular methods pose a challenge: they require significant adjustment for each task, despite sharing common modules. 
%As an example, MOPA~\cite{mopa} recently demonstrated that a simple policy of random exploration combined with a navigation model defined for PointGoal Navigation, could effectively replace traditional maps and path planners. %This not only yielded comparable performance but also demonstrated significantly faster decision-making, owing to the simplicity of a forward pass on a pre-trained network compared to the intricacies of mapping and subsequent planning.

In this context, our paper introduces \approach\ (see Figure~\ref{img:teaser}), a LLM-based compositional model build upon a pre-trained PointNav policy and incorporating a \ac{vlfm} policy~\cite{vlfm} (specifically integrated through a modular component which could seamlessly accommodate for alternative exploration policies if needed). %(an high level description is visible in Figure~\ref{img:teaser})
The primary aim of the proposed approach is to extend the paradigm of VisProg \cite{visprog} into the immersive scenario of EAI, where the agents interact with and navigate through the environment. %, ensuring a more comprehensive evaluation and application of language models in dynamic scenarios. 
%\approach\ also integrates modules for semantic navigation oriented towards approaching objects or modules for image recognition during navigation. 
\approach\ also integrates diverse modules designed for visual navigation and question-answering tasks, resulting in a system that seamlessly addresses both challenges while achieving great performance without requiring any prior adjustments.
These modules complement the primitives necessary for searching specific objects within the environments. 
By providing a few in-context examples/programs that show how to tackle multiple task, \approach\ is capable of generalizing to the specific task at hand. This is facilitated by the \ac{llm}, which effectively combines the individual modules available within the \approach\ system.
%Commenti Luciano: 
% Dire esplicitamente che per risolvere i task noi dobbiamo comporre i vari moduli assieme
% Aggiungere degli itmezie con tutti i contributi del paper (ultima cosa finale dell'introduzione).
%By providing a few in-context examples/programs that show how to tackle multiple task, such as ObjectGoal Navigation, solely using the modules already available in \approach, the LLM learns to combine these modules into programs to address the task at hand. 

To demonstrate the flexibility of the proposed framework, \approach\ has been tested on three popular benchmarks: namely, \emph{i}) Open-Vocabulary ObjectGoal Navigation~\cite{ovon},  \emph{ii}) Multi-Modal Lifelong Navigation~\cite{goat-bench}, and \emph{iii}) Embodied Question Answering \cite{open-eqa, das2018embodied}. \approach\ demonstrated competitive results with the previous works, including zero-shot approaches. Notably, unlike previous approaches, our framework is capable of handling multiple tasks simultaneously without the need for task-specific adjustments. Additional experiments on simpler tasks, such as ObjectGoal Navigation~\cite{batra2020objectnav} and Instance-ImageGoal Navigation~\cite{krantz2022instance}, are provided in the supplementary material (Section \ref{sec:supp_experiments}).

%namely, \emph{i}) ObjectGoal Navigation~\cite{batra2020objectnav}, \emph{ii}) Instance Image Goal Navigation~\cite{krantz2022instance}, and \emph{iii}) Embodied Question Answering~\cite{das2018embodied}. \approach\ demonstrated competitive results with the previous works, including zero-shot approaches. Notably, in contrast to the previous works, all the integrated modules in our framework either require no training or come pre-trained on standard datasets, thus not requiring any fine-tuning on a specific task.
